TVConv: Efficient Translation Variant Convolution for Layout-aware Visual Processing

As convolution has empowered many smart applications, dynamic convolution further equips it with the ability to adapt to diverse inputs. However, the static and dynamic convolutions are either layout-agnostic or computation-heavy, making it inappropriate for layout-specific applications, e.g., face recognition and medical image segmentation. We observe that these applications naturally exhibit the characteristics of large intra-image (spatial) variance and small cross-image variance. This observation motivates our efficient translation variant convolution (TVConv) for layout-aware visual processing. Technically, TVConv is composed of affinity maps and a weight-generating block. While affinity maps depict pixel-paired relationships gracefully, the weight-generating block can be explicitly overparameterized for better training while maintaining efficient inference. Although conceptually simple, TVConv significantly improves the efficiency of the convolution and can be readily plugged into various network architectures. Extensive experiments on face recognition show that TVConv reduces the computational cost by up to 3.1x and improves the corresponding throughput by 2.3x while maintaining a high accuracy compared to the depthwise convolution. Moreover, for the same computation cost, we boost the mean accuracy by up to 4.21%. We also conduct experiments on the optic disc/cup segmentation task and obtain better generalization performance, which helps mitigate the critical data scarcity issue. Code is available at https://github.com/JierunChen/TVConv.

==> rebuttal/acc_throughput_memory.tex <==
\begin{figure}
    \newcommand \AccThrMemwidth{0.494}
    \centering
        \begin{subfigure}[b]{\AccThrMemwidth \linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebuttal/Acc_T1-cropped.pdf}
        \caption{Against \textbf{MLPMixer}}
        \label{fig:AccThrMem_a}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[b]{\AccThrMemwidth \linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebuttal/Acc_T0-cropped.pdf}
        \caption{Against \textbf{self-attention} variants}
        \label{fig:AccThrMem_b}
    \end{subfigure}
    % \hfill  
    
    \begin{subfigure}[b]{\AccThrMemwidth \linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebuttal/Acc_T3-cropped.pdf}
        \caption{Against \textbf{per-image} dynamic conv}
        \label{fig:AccThrMem_c}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[b]{\AccThrMemwidth \linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebuttal/Acc_T2-cropped.pdf}
        \caption{Against \textbf{per-pixel} dynamic conv}
        \label{fig:AccThrMem_d}
    \end{subfigure}
    % \hfill
  
    \begin{subfigure}[b]{\AccThrMemwidth \linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebuttal/Acc_PMem0-cropped.pdf}
        \caption{Highest peak memory $<$ 500MB}
        \label{fig:AccThrMem_e}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[b]{\AccThrMemwidth \linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebuttal/Acc_PMem1-cropped.pdf}
        \caption{Highest peak memory $>$ 500MB}
        \label{fig:AccThrMem_f}
    \end{subfigure}
    % \hfill    
    \vspace{-0.2in}
    \caption{TVConv strikes a better accuracy-throughput trade-off under a medium memory requirement compared to related works. Benchmarking are conducted on the LFW face verification with the MobileNetV2 main backbone. A 4GB Raspberry Pi 4B is used. We set the batch size as 1/2/4/8/16 and the number of threads as 1/2/4, and report the maximum throughput for each model. The peak memory is measured with input size [8, 3, 96, 96]. }
    \label{fig:AccThrMem}
    \vspace{-0.2in}
\end{figure}

==> tables/varied_atom.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{Architecture} &
  \multirow{2}{*}{Operator} &
  \multirow{2}{*}{MACs (M)} &
  \multicolumn{5}{c}{Accuracy across datasets (\%)} \\ \cmidrule(l){4-8} 
 &
   &
   &
  LFW &
  CFP-FF &
  AgeDB-30 &
  CALFW &
  Mean \\ \midrule
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}MobileNetV2 \\ ×0.1\end{tabular}}  & Depthwise & 22.47 & 94.18 ± 0.34 & 93.01 ± 0.40 & 79.10 ± 0.44 & 82.50 ± 0.59 & 87.20 \\
 &
  CondConv &
  22.99 &
  94.44 ± 0.33 &
  93.31 ± 0.51 &
  79.09 ± 0.49 &
  82.74 ± 0.71 &
  87.39 \\
 &
  WeightNet &
  22.80 &
  93.51 ± 0.46 &
  91.77 ± 1.05 &
  77.02 ± 1.01 &
  81.23 ± 1.25 &
  85.88 \\
 &
  DYConvDW &
  23.43 &
  94.15 ± 0.43 &
  93.35 ± 0.36 &
  79.14 ± 0.64 &
  82.54 ± 0.70 &
  87.30 \\
 &
  Involuton (g=2) &
  52.05 &
  94.48 ± 0.13 &
  92.84 ± 0.06 &
  78.46 ± 0.51 &
  82.61 ± 0.28 &
  87.10 \\
 &
  Involuton (g=8) &
  34.47 &
  93.32 ± 0.64 &
  91.87 ± 0.59 &
  76.79 ± 0.85 &
  80.76 ± 0.90 &
  85.69 \\
 &
  DDF &
  27.77 &
  93.50 ± 0.21 &
  92.49 ± 0.50 &
  77.74 ± 0.58 &
  81.13 ± 0.48 &
  86.22 \\
 &
  \textbf{TVConv (ours)} &
  \textbf{22.47} &
  \textbf{97.16 ± 0.11} &
  \textbf{96.49 ± 0.21} &
  \textbf{84.61 ± 0.20} &
  \textbf{87.37 ± 0.21} &
  \textbf{91.41} \\ \midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}ShuffleNetV2 \\ ×0.5\end{tabular}} & Depthwise & 31.95 & 96.76 ± 0.08 & 95.95 ± 0.08 & 83.87 ± 0.37 & 86.71 ± 0.44 & 90.82 \\
 &
  CondConv &
  33.35 &
  96.79 ± 0.20 &
  96.04 ± 0.11 &
  84.80 ± 0.29 &
  87.37 ± 0.30 &
  91.25 \\
 &
  WeightNet &
  32.21 &
  96.71 ± 0.19 &
  95.63 ± 0.46 &
  83.62 ± 0.11 &
  87.03 ± 0.50 &
  90.75 \\
 &
  DYConvDW &
  32.30 &
  96.76 ± 0.15 &
  95.54 ± 0.43 &
  83.99 ± 0.52 &
  87.06 ± 0.23 &
  90.84 \\
 &
  DDF &
  33.77 &
  96.32 ± 0.21 &
  95.10 ± 0.51 &
  82.77 ± 1.22 &
  86.30 ± 0.79 &
  90.12 \\
 &
  \textbf{TVConv (ours)} &
  \textbf{31.95} &
  \textbf{97.61 ± 0.22} &
  \textbf{96.99 ± 0.11} &
  \textbf{85.86 ± 0.49} &
  \textbf{88.5 ± 0.35} &
  \textbf{92.24} \\ \bottomrule
\end{tabular}%
}
\caption{Comparison against related operators.}
\label{tab:varied_atom}
\vspace{-0.1in}
\end{table*}
